Humanoid Locomotion and Manipulation: Current Progress and Challenges in Control, Planning, and Learning

Humanoid robots hold great potential to perform various human-level skills, involving unified locomotion and manipulation in real-world settings. Driven by advances in machine learning and the strength of existing model-based approaches, these capabilities have progressed rapidly, but often separately. This survey offers a comprehensive overview of the state-of-the-art in humanoid locomotion and manipulation (HLM), with a focus on control, planning, and learning methods. We first review the model-based methods that have been the backbone of humanoid robotics for the past three decades. We discuss contact planning, motion planning, and whole-body control, highlighting the trade-offs between model fidelity and computational efficiency. Then the focus is shifted to examine emerging learning-based methods, with an emphasis on reinforcement and imitation learning that enhance the robustness and versatility of loco-manipulation skills. Furthermore, we assess the potential of integrating foundation models with humanoid embodiments to enable the development of generalist humanoid agents. This survey also highlights the emerging role of tactile sensing, particularly whole-body tactile feedback, as a crucial modality for handling contact-rich interactions. Finally, we compare the strengths and limitations of model-based and learning-based paradigms from multiple perspectives, such as robustness, computational efficiency, versatility, and generalizability, and suggest potential solutions to existing challenges.

==> Karen_notes.tex <==
\paragraph{The trend of reinforcement learning}

Reinforcement Learning (RL), enhanced by modern deep learning toolchains and algorithms, has garnered significant attention in the field of robotics over the past decade. RL promises an effective way to learn motor skills through end-to-end policies that translate raw sensory input to actuation, executable in real-time, with minimal or no supervision during training and without the need for labeled data or a differentiable world model \cite{}. However, in practice, the success of RL often relies on informative representations for both observation and action, extensive reward engineering, curriculum learning design, and a vast amount of trial-and-error experiences (data) to estimate gradients. Consequently, using RL to train robots is almost never practical in the real world. This makes the sim-to-real gap the Achilles' heel of RL, significantly dampening its initial promise.

Despite efforts to address the sim-to-real gap, a systematic solution remains elusive. Domain randomization, system identification, and simulator customization are mainstream approaches to mitigate this gap, but these measures are often ad-hoc and case-specific. This is why imitation learning, leveraging limited but in-domain real-world data, has gained popularity while pure RL has arguably been abandoned by many.

Nevertheless, RL has been successfully applied to various areas of robotics, with notable success in quadrupeds, where the sim-to-real gap has been consistently overcome. How can we apply the lessons from quadrupeds to humanoids for optimal loco-manipulation while avoiding known pitfalls? The success story of quadrupeds hinges on new investments in infrastructure for affordable hardware and highly parallel physics engines, spearheaded by key players in the robotics community. It is also important to note that the problem of quadruped navigation uniquely utilizes RL's strengths and avoids its weaknesses. Similar to robot manipulators, quadruped benefit from an inherently stable dynamic system thus less sensitive to sim-to-real gaps due to dynamic differences. However, unlike manipulators, quadruped navigation problems do not need to reason about complex object shapes and poses, sidestepping the sim-to-real gaps due to appearance and geometric differences in complex environments. 

In contrast, humanoid loco-manipulation faces challenging sim-to-real gaps both in dynamics and appearances. Actions that lead to whole-body balance have to be explicitly computed at the low-level control loop and multimodal observations of the environment must be considered in the control policy. Advancing in humanoid hardware and developing physics engines that model contact more accurately will be crucial. Imitation learning from human demonstrations will also play a key role in overcoming the sim-to-real gap in manipulation tasks.

\paragraph{Imitation learning from human motion data}
Recent success in robot manipulation through human teleoperation with imitation learning demonstrated the great potential of using human motion for robot learning. With the advantage of similar morphology between the humanoids and humans, many researchers hypothesize that humanoids can learn motor skills directly by mimicking a large, diverse corpus of human motion data, instead of relying on expensive online human teleoperation. 

While this hypothesis is plausible, several practical considerations must be addressed before we look into scaling up the data collection efforts. The central question we must answer is which aspect of human motion we want robots to learn. Some humanoid tasks can be achieved by simply mimicking 3D human pose trajectories \cite{}, but loco-manipulation requires physical interaction with the environment, based on human observations of the surrounding. Therefore, the human data must not only teach robots \emph{what} humans are doing, but also \emph{how} and \emph{why} they are doing it. In contrast, current data acquisition methods that capture human joint poses only enable learning what humans are doing. To develop truly versatile and adaptive humanoids, human data should also include physical actions and multimodal observations paired with the joint poses, so that humanoids can learn the how and why from human motion data.
 
In addition to this more comprehensive definition of “human data”, we also must consider the distribution of the human motion dataset. Prior work shows that using teleoperation to directly obtain “in-distribution” training data is crucial. In contrast, using offline human motion data to train humanoids inevitably creates an embodiment gap both in observation and action spaces due to different body proportions, joint configurations, and mass distributions between most humanoids and real humans. Closing this embodiment gap requires retargeting, which involves mapping motion collected from a source skeletal model to a target one. Previous work in computer graphics and robotics has explored various retargeting strategies, such as matching joint poses \cite{}, contact points \cite{}, end-effectors \cite{}, and high-level tasks \cite{}. Developing systematic solutions for retargeting remains a critical topic for advancing humanoids. 

Recent research efforts in collecting 3D human motion data have surged in computer vision and computer graphics communities. Currently, there are two primary approaches for acquiring 3D human motion data: A) recording 3D kinematic trajectories (joint positions/angles) directly from mocap devices and B) reconstructing it from existing 2D videos. The former produces higher-quality data but is difficult to scale, while the latter leverages abundant internet-scale data but generates lower-quality data. 

Regardless of which approach, we argue that improving the quality or scalability of 3D human motion datasets is not the most pressing issue for advancing humanoids, because the 3D kinematic trajectories alone do not have enough information to train the robots for loco-manipulation tasks, no matter how good or how big the dataset is. Instead, more research efforts should focus on human data that include corresponding egocentric observations and kinetic information such as joint torques and external forces. Recent works on collecting human multimodal observations \cite{} and human kinetics \cite{} are a few examples that aim to bridge the gap between human animation and humanoid applications. Together with the rapid advancement in humanoid hardware, imitation learning with more informative human data will become the mainstream approach to achieving versatile and generalizable humanoids.

% Removed from the main.tex
% Nevertheless, RL has been successfully applied to various areas of robotics, with notable success in quadrupeds, where the sim-to-real gap has been consistently overcome. How can we apply the lessons from quadrupeds to humanoids for optimal loco-manipulation while avoiding known pitfalls? The success story of quadrupeds hinges on new investments in infrastructure for affordable hardware and highly parallel physics engines, spearheaded by key players in the robotics community. It is also important to note that the problem of quadrupeds uniquely utilizes RL's strengths and avoids its weaknesses. Quadrupeds benefit from an inherently stable dynamic system similar to manipulators, while operating in a simplified and easily observable environment designed for quadruped locomotion. Due to the smaller size and limited manipulation capability  (often equipped with only a single arm) of quadrupeds compared with humanoids, quadrupeds' operating environment often involves a smaller space, and the environment uncertainty mainly comes from the terrain. Their tasks are largely focused on locomotion and possibly with simple manipulation tasks, which are highly different from human-like tasks that can be achieved by humanoids. As such, quadrupeds enjoy a robust basin of attraction less sensitive to sim-to-real gaps due to dynamic differences and the simple tasks they perform sidestep the sim-to-real gaps due to appearance and geometric differences in complex environments. 

% In contrast, humanoid loco-manipulation faces challenging sim-to-real gaps both in dynamics and appearances. For the gap in dynamics, actions that lead to whole-body balance have to be explicitly computed at the low-level control loop. For the gap in environment appearance, multimodal observations of the environment can induce significant sim-to-real gaps, such as lighting conditions, weather, and surface texture. These observations may cause instability in the control policy. Advancing in humanoid hardware deployment and developing physics engines that model contact more accurately will be crucial. Imitation learning from human demonstration or experience will also play a key role in overcoming the sim-to-real gap in loco-manipulation tasks and will be introduced.} 

% \Karen{The two paragraphs above can be condensed. My original text does not consider the quadrupeds with manipulation. It does not make sense to extend the original text to include quadruped manipulation. I'd just simplify the discussion to avoid potential arguments from reviewers. Here is a simplified version for the two paragraphs. }




% Can we also answer this question: how can versatile human motions in graphics be achieved on a real humanoid robot? Suggesting new promising methods to readers and concluding the main trend in the near term would be valuable.


==> deleted_txt.tex <==
Humanoid robots executing loco-manipulation tasks hold tremendous potential. There still remain numerous open questions. We hold hope that the humanoid robot will become a general workforce that transforms the world and benefits people from all areas.


\subsection{Dual-arm Manipulation}

Does a robot need dexterous hands? A swappable hand-like tool change. heavy duty vs dexterous. Hand and foot design may be interesting. 

Dual-arm manipulation systems, known for their versatility and dexterity, significantly outperform single manipulators by offering increased efficiency, precision, and success rate. The goal of dual-arm manipulators is to achieve universal manipulation, i.e., manipulating arbitrary objects with various geometric and physical properties \cite{dual_arm_TRO}. However, the key advantage of dual-arm manipulator systems in terms of manipulation dexterity is far from being fully exploited since arm cooperation is missing \cite{dual_arm_TRO}.

In order to achieve universal manipulation, researchers have been focusing on universal grasp generation and safe motion planning. The universal grasp generation focuses on generating a grasp for arbitrary objects. Motion planning focuses on generating a safe, collision-free trajectory to reach the target grasp. 

Although the arm and leg design for humanoids has largely converged, the dexterous hand design for humanoid robots is yet a hanging topic. The majority of humanoid robots nowadays are equipped with no gripper or parallel jaw grippers. Only a few robots are equipped with grippers with more than two fingers and actually leverage the extra dexterity. To determine the proper design for the hand, a necessary first step is to define the list of manipulation tasks the robot should achieve. However, no benchmark (list of tasks) or analytical metric has been proposed to evaluate the performance that can be achieved with these gripper designs. 
As an overall goal, the end-effector should provide strength and dexterity: a trade-off between lightweight and sturdy, given the price constraint. 
Several companies are designing dexterous hands that closely mimic human hand structure, which we argue may not be the best hand design. This multi-finger design introduces unnecessary mechanical complexity and end-effector weight, and its delicate structure can cause maintenance issues. It also introduces complicated sensing and control problems. For example, \cite{sferrazza2024humanoidbench} showed that the state-of-the-art RL policies fail to train proper humanoid behavior, given the extra DoF from the dexterous hands lumped into the state space. On the other hand, a parallel gripper relying on fingertips can be less effective in generating a firm gripper for heavy weights, such as cutting a knife or holding a chair. 
Three-fingered grippers, as shown in Fig.~\ref{fig:gripper_designs}(b), could be a sweat spot that embraces the advantages of both worlds. %However, the optimal design should be defined by the task we want to achieve. It is not clear right now what is the task set for the humanoid bi-manual manipulation.


When handling heavy objects, humans can naturally use multiple body parts to brace them or leverage external supports such as a wall \cite{SR_manipulation_learning_survey}.


The robot hand design is still a hanging topic, as most humanoid robots nowadays have no hand or parallel jaw grippers. 
While the arms and legs of humanoid robots have largely converged to anthropomorphic design, it is not certain if anthropomorphic robot hands are the way to go. 
On one hand, by mimicking human hands, it is guaranteed that the best result will be a general end-effector that can do whatever humans do. It is also easier to directly use human manipulation data to train the hand manipulation policy. 
On the other hand, control and planning complexity, cost, and maintenance effort are much higher for more complex hands. Currently, we also do not have good references or benchmarks to test how general a robot hand needs to be for daily manipulation. It is possible that simpler hands can also achieve similar functionality. A final question is, why are human hands so dexterous? One main reason is tool-using. If so, why not let the robot have a quick tool changer system that can switch to different tools quickly?




Although the arm and leg design for humanoids has largely converged, the dexterous hand design for humanoid robots is yet a hanging topic. The majority of humanoid robots nowadays are equipped with no gripper or parallel jaw grippers. Only a few robots are equipped with grippers with more than two fingers and actually leverage the extra dexterity. To determine the proper design for the hand, a necessary first step is to define the list of manipulation tasks the robot should achieve. However, no benchmark (list of tasks) or analytical metric has been proposed to evaluate the performance that can be achieved with these gripper designs. 
As an overall goal, the end-effector should provide strength and dexterity: a trade-off between lightweight and sturdy, given the price constraint. 
Several companies are designing dexterous hands that closely mimic human hand structure, which we argue may not be the best hand design. This multi-finger design introduces unnecessary mechanical complexity and end-effector weight, and its delicate structure can cause maintenance issues. It also introduces complicated sensing and control problems. For example, \cite{sferrazza2024humanoidbench} showed that the state-of-the-art RL policies fail to train proper humanoid behavior, given the extra DoF from the dexterous hands lumped into the state space. On the other hand, a parallel gripper relying on fingertips can be less effective in generating a firm gripper for heavy weights, such as cutting a knife or holding a chair. 



\subsection{Humanoid design}
The mechanical design of humanoid robots remains an open space for improvement. We list several interesting points in this section.

Leveraging joint coupling mechanisms in leg design could allow an extended range of motion, augmented joint outputs, and more strategic placement of joint actuators \cite{perera2024staccatoe,sim2022tello}. However, achieving such a design may be challenging and overwhelming due to the wide selection of hardware components and transmission techniques. \cite{sim2023control} explores the possibility of streamlining this process through structured optimization problems. Topology optimization is a great tool to optimize the link shape, keeping a balance between structure rigidity and weight \cite{zhu2023design}.

Humans are energy efficient when standing because a straight knee at a fully extended configuration is locked, known as the screw-home mechanism. A self-lock mechanism of the knee \cite{screw_home_knee} and ankle \cite{lock_ankle} helps leverage mechanical structure rather than motor torque to provide support.



% Parallel linkage transmission designs are popular and robust approaches on many humanoid robots. However, due to the four-bar parallelogram geometry, the design has to balance between compactness, mechanical robustness, and range of motion. In addition, the inherent mechanical contact noise may not be ideal for certain applications.  

Hollow shaft joint actuators have become an emergent design choice on many recent humanoid robots (e.g., New Atlas, Unitree H1, and G1). They expand the range of motion and mitigate wiring-induced failures in complex scenarios that require extreme joint angles. 

Designing for compactness and self-folding is another design factor that allows humanoid robots to fit in human-oriented workspaces. Transportability is an important design for users and developers to fit the robot into a box or a car.


Arm movement not only improves walking stability but also reduces the overall control effort \cite{arm_swing_worth}. 


% \ZGU{swappable hand: using the best tool for the right task. }
The robot hand design is still a hanging topic, as most humanoid robots nowadays have no hand or parallel jaw grippers. 
% While the arms and legs of humanoid robots have largely converged to anthropomorphic design, 
It is not certain if anthropomorphic robot hands are the way to go. 
On the one hand, by mimicking human hands, it is guaranteed that the best result will be a general end-effector that can do whatever human hands can do. It is also easier to directly use human manipulation data to train the hand manipulation policy. 
On the other hand, design and manufacturing difficulty, control and planning complexity, cost, and maintenance effort are much higher for more complex hands. 

In order to have a design that is actually useful for the task of interest, a general benchmark system and evaluation metrics need to be proposed. Currently, we also do not have good references or benchmarks to test how general a robot hand needs to be for daily manipulation. It is possible that simpler hands can also achieve complex functionality for daily manipulation. 

If we ask the question, ``Why did humans evolve dexterous hands?''. One main reason is tool-using. From a tool-using perspective, it is an effective strategy for humanoid robots to have swappable end-effectors, such as the automatic tool changer system in computerized numerically controlled (CNC) milling machines. Therefore, instead of having a dexterous hand to manipulate the tool, a tooled end-effector is much more reliable. %If so, it might be more efficient to have the robot end-effector be a quick tool changer system that can switch across to different tools.

\begin{figure}\centering
\includegraphics[width=0.48\textwidth]{figures/grippers.pdf}
\caption{
Common hand design for humanoid. In order to achieve dexterity and sturdiness, the hand needs to generate prehensile force. 
(a) Psyonic's ability hand; % https://www.psyonic.io/
(b) Robotiq's three-finger gripper; % https://robotiq.com/products/3-finger-adaptive-robot-gripper
(c) Strunk's parallel gripper. % https://schunk.com/us/en/gripping-systems/parallel-gripper/mpg-plus/c/PGR_3060
}
\label{fig:gripper_designs}
\vspace{-0.15in}
\end{figure}

\subsection{Learning Loco-Manipulation Skill from Scratch}
% \ZGU{Combining RL learning with search is a promising direction, as proved by the success of alphaGo, which achieved superhuman performance leveraging MCTS with RL. \cite{}
% }

\section{WBC}
For example, if the desired CoM acceleration is $20$ m/s$^2$ in the direction of gravity, no torque is able to pull the robot down at this rate if contacts are unilateral (nonsticking). But if the robot tries to launch off the ground from a double stance configuration, there can be infinite combinations of ground reaction forces to achieve this, as long as their sum overcomes gravity. 

Another limitation lies in its reliance on instantaneous, reactive control, which tends to be myopic. A recent trend in whole-body control is to expand the horizon of the WBC, effectively making it an MPC. Of course, this pays the price of losing convexity, as the dynamics constraint between the future states and the current state is non-linear. With recent success in speeding up MPC, this is a promising direction with much more new research to come. 
This NLP has been historically hard to converge in real-time. It is typically solved via sequential quadratic programming. Recent studies \cite{Galliker2022PlanarBL} achieved real-time whole-body MPC by solving only a few iterations and stopping the solver pre-maturely. The whole OCP will restart with the latest measurement and use the previous trajectory as a warm start. The rationale for this basin-of-attraction lies in the nature of MPC, the prediction is outdated when you take time trying to converge to an optimal solution. The best thing you can do is to retrieve the latest state, which is the only thing relevant at the moment, before continuing solving. This method has mostly been put into practice for DDP-based MPC \cite{WB_MPC_Dantec} because the roll-out trajectory all always dynamically feasible. Still, it is common practice to provide a good initial guess  (an offline converged solution) to warm start the very first problem.

For example, to track a dynamic walking motion from an MPC, this QP framework includes a contact task for the stance foot and a trajectory-tracking task for the swing foot. Additionally, the task for the torso tracks a centroidal trajectory of the motion. 

Pre-calculated parkour movement can also be executed robustly with the WBC controller. The contact forces can be addressed and utilized to reach the desired shifts in centroidal momentum.

One of the limitations of these optimization-based WBC is the lack of robustness against sudden changes in the constraint set. Fast and accurate contact detection is key because the QP is brittle from inaccurate contact estimates. In this sense, tactile sensing across the robot's body \cite{wholebody_tactile} proves beneficial. Similar to human skin, it enables the detection of unforeseen collisions or contacts and facilitates the redistribution of joint torque to accommodate these contacts.

The resolution of dynamic tasks can be solved efficiently (at most on the order of milliseconds) when formulating WBC as a quadratic program (QP). 

Dynamic tasks are represented as equality or inequality linear constraints. %:
$$
A\boldsymbol{X}-b=\boldsymbol{s_e}, D\boldsymbol{X}-f \leq \boldsymbol{s_{ie}}
$$
This general task representation captures various behaviors, such as CoM trajectory tracking, moving a frame to a certain pose, or maintaining contact. 
For hard constraints, the slack variables $\boldsymbol{s_e}$ and $\boldsymbol{s_{ie}}$ will simply take zero. Otherwise, their square of norm can be added as a quadratic cost term. Such task structure grants versatility, as it can describe varied behaviors simply by adding or removing tasks. 


, which offers a significant advantage: it converges to an optimal solution when multiple solutions are possible, and finds the least violating solution when no exact solution is achievable.

\section{Multi-Contact Planning}
Loco-manipulation has been successfully demonstrated on quadruped robots with an arm \cite{sleiman2023versatile, sleiman2021unified, rigo2023hierarchical} as well as leveraging only body contacts \cite{wolfslag2020optimisation, sombolestan2023hierarchical, rigo2023contact,arm2024pedipulate}.
Real-time contact-implicit planning on quadruped locomotion has also been achieved in \cite{kim2023contact, le2024fast}. 

Multi-contact planning is still one of the most challenging tasks in robotics. In the context of humanoid whole-body loco-manipulation, the planner aims to solve trajectories involving contact interactions with environments or objects. Due to the underactuation nature of humanoid robots, contact is critical for maintaining balance. Due to the environment or object having diverse physical properties (e.g., rigid or soft, fixed or movable), this type of problem is inherently contact-implicit; the planner needs to make decisions on contact locations, contact timings, and contact force. 
Preliminary results on humanoid loco-manipulation planning have been demonstrated in the past decade, showcasing promising potential in many different multi-contact tasks, such as \cite{lengagne2013generation, ponton2016convex, vaillant2016multi, henze2016passivity, tsagarakis2017walk}.
However, there remains an open problem on how to use contact-implicit planning to achieve efficient and natural multi-contact whole-body loco-manipulation behaviors on humanoids.
Whole-body manipulation leverages whole-body poses and contact of body parts to aid object manipulation, as shown in Fig.~\ref{fig:human-loco-manipulation}. 
However, it requires solving meticulous and high-dimensional planning problems to generate such contact and pose sequences for humanoid robots due to the uncertainty of contact and modeling of highly complex robot dynamics. 

Preliminary results in humanoid multi-contact planning have been demonstrated. For instance, Atlas humanoid \cite{BD_gymnastics} uses its curvy back to roll on the ground. HRP-4 humanoid leans against the box to maximize push force \cite{Murooka_heavy_push}. Walk-man humanoid uses hand contact with the wall during door-opening tasks to assist balance \cite{tsagarakis2017walk}.
In these loco-manipulation applications, due to the increasing demands of online planning in the control system structure, the real-timeliness and efficiency of these techniques are highly sought after. 


Numerical optimization-based methods such as model predictive control (MPC) and direct trajectory optimization (TO) impose contact constraints implicitly in the problem formulation to solve for contact sequences, contact locations, contact forces, and robot trajectories via gradient-based optimization methods \cite{ferrari2023multi,ruscelli2020multi,lee2021efficient,ferrolho2023,sleiman2019contact, kurtz2023inverse, le2024fast}. 
Unlike TO problems, which are meticulously designed and are typically solved offline, MPC-based approaches often use reasonable model simplifications and solver-level improvements to enable efficient online computations.
However, employing high-dimensional full-body models remains computationally expensive. This inherent computational burden is likely to remain a bottleneck for real-time control for the foreseeable future \cite{Wensing_survey_TRO}.
Although there presents a quite limit body of work of real-time CITO on humanoid robots,  recent attempts has proven viable options in speeding up CITO, including reasonable dynamics and contact modeling simplification and trading off certain solution accuracy for computation efficiency. \citet{Dai_centroidal_kinematics}
uses kinodynamic modeling instead of whole-body dynamics on humanoid robots for contact-implicit planning.
While optimization-based methods have traditionally been limited to offline trajectory generation due to their heavy computational burden, recent advancements in optimization techniques have significantly accelerated computation speeds.
The whole problem can be formulated as a single nonlinear programming (NLP), which is better than traditional MIP, but is ill-posed. 
\ZGU{Comment on whether the state-of-the-art can solve realtime? How about using high-dimensional full-body dynamics?}
(mention contact-implicit optimization requires complementarity constraints as contact constraints, refer to \cite{MPC_survey})


\subsection{Manipulation for Humanoids (or Anthropomorphic Manipulation?)}

\subsubsection{Dual-arm Manipulation}
Dual-arm or bimanual manipulation is mostly motivated by its anthropomorphic characteristic --- the robot systems having two arms like humans. Dual-arm systems have several potential advantages over single-arm systems~\cite{smith2012dual}. First, the anthropomorphic similarity enables more intuitive and easier transferring of skills from humans to robots. Second, two robot arms have more degrees of freedom, providing enhanced flexibility and manipulability. Third, dual-arm systems provide two grasp to the object, therefore providing more strength and better object handling, enabling many tasks in daily life involving large, heavy objects that can only be handled with two arms, such as holding a fire hose and lifting a table. Additionally, the human-like dual-arm setups also potentially facilitate human understanding and human-robot collaboration. 
Compared with single-arm manipulation, dual-arm manipulation is featured by the space and temporal coordination of the two arms, and physical interactions and force transmission of the two hands~\cite{smith2012dual}. 
The three challenges are unique in dual-arm manipulation. 
1) Due to the high dimensionality of the degrees of freedom of the two arms, motion planning suffers from exponential computational costs.
2) The coordinative and contact-rich nature of dual-arm manipulation requires compliance in control. It often requires nontrivial switching strategies between different control modes. 
3) The complexity of dual-arm manipulation requires a better understanding of human manipulation.  
4) For humanoids, dual arm motion generation is even more difficult as it requires the consideration of balance, taking into account the object's effect on the floating-based robot. 

Recent works in dual-arm manipulation systems have diverged in two directions: the model-based direction and the learning direction.  
In the model-based direction, \cite{dual_arm_TRO} integrated learning for bimanual grasping generation, self-collision avoidance planning, and online cooperative manipulation, achieving coordinated, compliant dual-arm manipulation in tasks like rearrangement and turnover manipulation. \cite{krebs2022bimanualtaxonomy} proposed a taxonomy that emphasizes the coordination and interaction of bimanual manipulation, contributes to a better understanding of human bimanual manipulation, and potentially helps guide the development of robot systems.  
In the learning direction, the motion planning and control scheme are replaced by pure learning techniques. \cite{chen2022towards} developed a Bimanual Dexterous Hands benchmark, with the goal of using reinforcement learning to match human-level skills with reinforcement learning. \cite{aldaco2024aloha} developed a low-cost leader-follower dual-arm system that leverages human demonstration to perform imitation learning. 
Despite the recent progress, the key advantage of dual-arm manipulation systems in terms of manipulation dexterity still needs to be fully exploited, since arm coordination and interaction are still at a preliminary stage for contact-rich tasks.

\subsubsection{Whole-body Manipulation}

Humans can make use of any part of our bodies to manipulate objects. For example, we use our palms or fists to provide large forces. We use our elbow or hip to hold a door open for convenience. In comparison, most robot arms often have predefined end-effectors, which are the only parts designed to interact with the world. 

The idea of using the robot links to manipulate is originally proposed as whole-arm manipulation in \cite{salisbury1987whole}. Whole arm manipulators (WAM) were originally designed and built to explore the benefit of manipulating objects with all surfaces of a robot manipulation \cite{townsend1993mechanical}. 
More recently, Punyo, a robot made with soft materials and full body sensing, aims to provide whole-body manipulation capability in a build-in manner \cite{goncalves2022punyo}. 
Researchers also studied this problem as whole-limb \cite{bicchi1994problem} or whole-hand manipulation \cite{vassura1993whole,pollard1994wholehand}. 

The dynamics and control for whole-arm manipulation are studied in \cite{song2000dynamic} \cite{song2001dynamics}. Due to the existence of passive reaction forces, the force distribution problem is examined in \cite{bicchi1993force,haas2021grasp}. 
Planning and control of whole-arm manipulation are also studied.
Contact states and transitions are used to plan whole-arm manipulation object motions for whole-arm in-hand manipulation \cite{trinkle1991framework, trinkle1993dexterous, watanabe2006towards, yamawaki2013randomized}. 
\citet{hsiao2006imitation} used teleoperation and imitation learning to synthesize object grasping motions considering the whole robot body. 
With reinforcement learning techniques, 
\citet{yuan2019reinforcement} learns to generate whole-arm motions for holding and transporting humans in rescue scenarios, and \citet{zhang2023plan} enables the Punyo system to move large objects guided by planning.  

Despite the progress made by the previous work, unsolved challenges are still present in whole-body manipulation. Most of the research focuses on whole-arm manipulation with the upper limb. The ability to use all usable body parts has yet to be developed. In addition, it remains unknown how to achieve this complex behavior of whole-body manipulation, which requires planning, control, and sensing of every point on the robot. 

\subsubsection{Dexterous Hands}

Although the arm and leg design for humanoids has largely converged, the dexterous hand design for humanoid robots is yet a hanging topic. The majority of humanoid robots nowadays are equipped with no gripper or parallel jaw grippers. Only a few robots are equipped with grippers with more than two fingers. However, due to the complexity of dexterous manipulation, the extra degrees of freedom for dexterous hands are often not fully leveraged, and most of the dexterous hands are still only used for grasping. 

Most of the time, the design goal is to mimic a human hand, which has 22 DoFs \cite{}.
However, mimicking human hands is not trivial. \cite{} ..., which is the closest to human fingers and hands. But the design, fabrication, and maintainance are complicated and not easy to be replicated. Most of the existing dexterous hands, while mimicking the appearance of human hands, has much less DoFs. Examples: Allgero hands, Shadow hands, Leap hands, the hands in Nancy Pollard's groups, the early hands...
If we think about the mechanisms of machines and humans, they are essentially different. (talk about human mechanism and machine mechanism.) 
In addition, the complexity of planning and control of dexterous hands is great. There are so many DoF, self-collision, and compliance of hands. Essentially, this is a trade-off of ... 
In addition, we are not sure if human hands are the optimal structure for manipulation. 

Considering the limitations mentioned above, perhaps it is worth asking the question, is our design goal of mimicking the appearance of human hands really what we want? Instead of mimicking the kinematic structure of human hands, it is worth considering mimicking the functionality of human hands. However, we have not seen any metric or task set to functionally guide the design of dexterous hands. We expect to see future work in benchmarking the design of dexterous hands in mimicking human hand functions, co-design approaches for hands, and enabling cross-morphology adaptation of robot hands in dexterous manipulation. 

\subsection{Data Scarcity}
When the brain-robot interface technology becomes mature, we will be able to control the robot with our brain signals. Recording the brain control signal might be a great way to quickly get abundant and rich data. (This is too sci-fi, is this really supported by any research?)


However, it is not clear how relevant datasets learned on YouTube can generalized to humanoid robots.

The best quality demonstrated data comes from model-based methods or reinforcement learning because there is only a small gap at deployment after training. The data include the sensory input and actions while the humanoid robot performs the desired task. However, unlike the ubiquitous robot manipulators, datasets collected directly from humanoid robots are not openly available, due to the lack of deployed humanoid robots. Collecting large datasets of humanoid skills is slow and expensive. It often requires meticulous engineering to get adequate data for even one skill, all while guaranteeing safety along the process. Using simulation to parallelize can accelerate the data collection \cite{Orbit}. However, the fidelity of the simulator will inevitably cause a sim-to-real gap.

To address this issue, teleoperation is another way to get robot data that is close to the robot morphology. However, it also involves significant human expertise to achieve successful robot execution. Also, it is not trivial to build a teleoperation system that can map both locomotion and manipulation skills from humans to humanoid robots \cite{teleop_humanoid_review}. 

Human demonstrations are more available because it is more intuitive for humans to demonstrate directly than to distill human knowledge by laying down reward designs or tuning controller hyperparameters. Several endeavors have been attempted to collect large-scale human mocap data \cite{KIT_wholebody, AMASS}. Motion capture data are a great proprioception data source. However, tactile feedback and actuation will not likely be retrieved from human demonstrations. %Due to the close resemblance between humans and humanoids, these demonstrations can be retargeted to humanoid robots. Being able to leverage human demonstrations is one of the reasons that humanoids are fundamentally better than other form factors.

What is the data that we need? How diverse, How large is the dataset, and what information should the data contain? If I want to create an open-source dataset, what do I need to prepare for others? How do we consider the different form factors between robots?

On the road toward generalist humanoid robots, humanoids are limited not by their physical capability but by the scarcity of robot data. 
However, for any new tasks, new environments, or new robots, recollection of a dataset is required. Therefore, the scarcity of data has always been a significant bottleneck in robotic skill learning
Indeed, first-hand robot data across every object, environment, and task is a limiting bottleneck.
For humanoid robotics, the limited dataset is caused by the limited number of humanoid deployments, a chicken-and-egg problem. 

\subsection{Loco-manipulation}
Although agile movements such as parkour \cite{humanoid_parkour_learning} or gymnastics \cite{BD_gymnastics} seem irrelevant to the HLM application, these tasks represent underlying technologies that are relevant and important for the HLM applications. (i) Even though the majority of the humanoid task is slow, steady movement, the humanoid robot's inherent unstable dynamics will require the robot to perform fast recovery motions from time to time. The robustness of the robot is critically dependent on the dynamic whole-body movement in order for this system to have long robust operating hours. (ii) The parkour and gymnastic movements are the indicators of whole-body dynamic balancing ability, which involves coordinating legs and arms to maintain balance, exerting a huge wrench on the ground to accelerate the system, and, most importantly, accurate estimation of the system state.


\subsection{Generalization and Scaling for Humanoid Deployment}
A recent trend in robotics works towards training “generalist” robot policies on large diverse robot datasets. 
Generalization is the ability to apply learned skills or knowledge to novel scenarios, tasks, or embodiments. This ability is crucial for the mass deployment of humanoid robots. 
Many algorithms focus on imitation policy that provides one-shot generalizations to novel objects and tasks \cite{Finn2017OneShotVI} and zero-shot generalizations to new objects and scenes \cite{jang2022bcz}. These systems are conditioned on learned task embedding, which can be encoded from language instruction or video demonstration. 
% Humanoid robots are built with generalization in mind. They are expected to achieve diverse human-level tasks. 
% However, most of the traditional methods are engineered for a specific task in a specific environment. For example, RL can learn many skills. Imitation learning also learns the set of skills within the demonstrated dataset. But they lack the ability to generalize,  performing new skills in a new environment with minimal further training \cite{}. 
% \subsubsection{Generalization in Novel Skills}


% Some will shuffle the dataset to mix in old data when adapting to a new environment. 
%However, both methods will plateau when the dataset keeps expanding. Humans, on the other hand, don't require significantly fewer training samples to learn a certain skill, such as moving a box. There might be a totally different paradigm that leads to the generalist agent, such as the world model \cite{world_model_lecun}.


\subsubsection{Generalization in Novel Environment}
Domain adaptation involves adapting existing skills to a real-world environment. 
% Since the trained policy needs to be deployed in diverse environment setups and have close interaction with novel objects, the ability of the policy to adapt motions to these novel geometries is important. 
One of the naive ways to solve this problem is to randomize the object and environment setup to exhaustively enumerate all possible environments during training. But this is challenging as it explodes the data. \cite{neural_state_machine}

\subsubsection{Generalization in Novel Task}
Leveraging existing skills to solve new tasks. Many networks will adapt to new tasks but forget the existing skills \cite{}. 
Transfer learning uses a policy learned on one task to train a learner on another task. \ZGU{Imitate and repurpose paper.} \cite{driess2023palme} show positive transfer, where scaling the foundation model size and training data enables fine-tuning with less catastrophic forgetting. 
Continual learning, being able to continue expanding the skillset is a key capability of a generalist agent. Robotcat \cite{} is one such method.
Octo trains a generalist policy that can control multiple robot zero-shot and allows efficient fine-tuning for new robot \cite{Octo}.

\subsubsection{Generalization in Novel Robot}
Humanoid robotics, although they mimic human shapes, are built with different sensors and have different kinematic and dynamic properties. \cite{bousmalis2023robocat} is a foundation model based on the generalist agent Gato \cite{reed2022generalist}. It is able to collect data on new robots and continuously improve its task success rate across different morphology. 

In the following section, we discuss the potential of foundation models in achieving generalist robot agents.


\textit{NMPC Speed-up via Solver-level Improvement:}
Sparsity in QP matrices can be utilized. Solving the Newton step inside optimization will almost always require solving the linear KKT equation. Solvers like OSQP and qpSWIFT utilize graph-based Cholesky Factorization to accelerate this computationally expensive step, by only considering the non-zero elements inside the matrix.
A memristor-based analog QP solver is introduced in \cite{cheng2023memristor} to reduce the computation latency by 2000 times. 
This work can be further developed to accommodate and accelerate nonlinear SQP problems in complex loco-manipulation planning problems. 

\subsection{Opportunities and Challenges in Foundation Models}

Foundation models cannot solve Moravex's paradox yet. Enabling FMs to directly command robot action is challenging, with only a few successful studies. 
The vast majority of the current research uses foundation models as a task-planning module because it does not require expensive pre-training. 
In the near term, training foundation models using robotics data will continue to be difficult and will be available only to companies with computation resources. Closer collaboration between industry and academia will be important to continue to push forward in this area.  

Due to limited physical knowledge and hallucination effects, some middle-level behaviors are inadmissible based on unrealistic knowledge.
Regulating the output of the foundation models is an active research area. %LLM has a hallucination effect that produce infeasible plans and unrealistic knowledge. 
In such cases, a supervision system that provides feedback to the robot is critical. A low-level policy that reports infeasibility will increase the task success rate. Also, LLM cannot plan novel actions \cite{kambhampati2024llms}. They produce plans only because they have been trained with this plan in the dataset. 

Restricting the LLM's output to an existing set of skills is also a common approach \cite{saycan}.
To refine the foundation model's output to appropriate skills, grounding strategies such as prompting actionable skills or evaluating skills through affordance \cite{saycan2022arxiv} are employed.

However, a humanoid foundation model is yet to exist. The lack of humanoid data is one of the primary hurdles for training a humanoid foundation model. Data acquisition and training/fine-tuning is prohibitively costly. Most of the available datasets are for single-arm manipulation tasks. %Due to the lack of such data, human demonstrations, either recorded or from the internet, would be a valuable source. Teleoperation systems would also be necessary to speed up the data collection, although the availability is much more limited than human demonstrations. 

\subsubsection{Long-Horizon Task Planning and Task-aware Re-planning}
To execute tasks robustly, the policy needs to be aware of the task execution progress and success rate. If the robot fails at one point, the planner needs to use multi-modality sensors to understand the state of the task and execute and re-try the task execution if the task fails.

\subsection{Pure RL}


To avoid these problems, the majority of robot learning algorithms leverage demonstration or experience for effective training.

However, RL methods may achieve one specific task via simple heuristics or reward tuning. These heavily-engineered skills cannot generalize to new skills and, therefore, are difficult to adapt to diverse unseen environments, making them far from becoming a generalist policy.

The policy deployment often exhibits a significant gap due to model mismatch between the simulation and real hardware. Furthermore, the sparse nature of reward design often hinders effective policy exploration, necessitating meticulous expert tuning. 


\section{Applications of Humanoid Loco-manipulation}
\label{sec:application}

The application of humanoid robots is multifold. Some tasks involve non-physical demanding tasks such as telepresence, question answering, and navigation assistance. Most of the tasks require physical skills. These tasks are complex as they involve rich physical interactions with the environment, such as object pick-up and delivery, tool and facility operation, and navigation.
This section focuses on the physical tasks involving loco-manipulation capability and talks in-depth about two specific applications: manufacturing and human-humanoid collaboration. 

% In the short term, the application of humanoid robots would be simpler tasks, where the robot has a fully defined routine in a structured environment, such as autonomously completing a task in a manufacturing factory or a warehouse logistics. This is what many humanoid robot companies and car manufacturers see opportunities in as they are teaming up to accelerate the deployment. 
% In the long term, as humanoid robot's capability generalizes, the robot may work in unstructured environments and work collaboratively with humans. Such examples are interactive care services and household assistance. %Recently, grounding foundation models on humanoid robots achieved long-horizon task planning and execution. For example, \cite{MenteeVideo} has shown the capability of humanoid robots to take verbal commands and execute complex tasks, including navigation in office space, locomotion, semantic understanding, object detection, localization, manipulation, and natural language understanding.

\subsection{Human-Humanoid Interaction and Collaboration}
% \ZGU{check: Human-humanoid interaction and cooperation: a review}

Human-humanoid collaboration is still in its infancy, with some applications in dancing \cite{tactile_dance} and collaborative object transportation \cite{HRP-table-collab}. 

Several challenges lie in collaboration tasks. First, developing cognitive interaction skills such as verbal, visual, and physical signals to effectively capture human cues and their intentions~\cite{vianello2021human}. Second, how to make decisions with situational awareness and human-in-the-loop communication and task adjustment~\cite{romano2017codyco}. Third, safe motion planning and control for humanoid robots is a non-trivial problem when considering collision avoidance in environmental navigation, force interaction with the object, and foot placements to maintain balance~\cite{otani2018generating}. Several studies estimated human information and incorporated it into low-level control. The study in \cite{romano2017codyco} proposes a human-aware whole-body controller. They estimate the human state through sensors attached to the human and predict the human's intentions through dynamic quantities such as torques and accelerations. This human-centered information is used to develop a balancing controller that exploits the support the human offers. The authors in~\cite{otani2018generating} present a real-time multi-robot quadratic program that models both the human and the robot whole body dynamics. The controller archives co-manipulation tasks and maintains balance for the robot, however it is only demonstrated in simulation.

Collectively lifting and transporting heavy objects is of particular interest as it is a common skill. The collaboration can happen either between humans and humanoids or between a team of humanoids. Collective transport strategies have been conventionally designed for grounded robots, aerial robots, and surface vehicles. However, it is largely underexplored for legged robots due to its complex underlying robot dynamics. Although some recent works explore collaborative transport with quadruped robots \cite{fawcett2023distributed, CMPC_locomanip}, these robots do not scale to human-robot teaming due to the different sizes and leg morphology between quadrupedal robots and humans. Given humanoid robots' anthropomorphic similarity to humans, they are well-suited to interact with humans~\cite{vianello2021human}. As they are built to resemble humans for ease of social acceptance and for functioning in environments designed for humans, they are particularly suited for accomplishing collaborative scenarios with humans. 

Another area of human-humanoid interaction is social navigation, which can serve as a form of virtual interaction. In social navigation settings, the humanoid is tasked to navigate a social environment, such as shopping malls or construction sites, while adhering to social norms and behaviors. In social navigation, the interaction is bidirectional, as the path taken by the human influences the path plan for the robot and vice versa. Social navigation is an active area of research~\cite{mavrogiannis2023core}. For instance, humanoid social navigation \cite{shamsah2024real, shamsah2024socially} explores socially acceptable path planning in reach-avoid tasks while obeying the dynamic feasibility of a humanoid robot.

\subsection{Manufacturing}

The humanoid robot can be a universal solution to the labor shortage issue as it can be generalized to diverse, repetitive, and even hazardous tasks. Being plagued by the labor shortage issue, car manufacturers are collaborating with humanoid start-up companies to build humanoids that can be deployed in the manufacturing factory. However, these factories are already highly automated by industrial robots. To find tasks that are handled by humans but cannot yet be automated by humans is highly difficult. 
% However, carrying is a human's unique superpower compared with other animals. Moving heavy objects is the hallmark of the humanoid's ability to be useful. Fig.~\ref{fig:A} should be the several ways that humanoids could be useful in moving objects around and become useful. 

One of the tasks unique to humanoid robots could be carrying heavy objects over to a mobile platform. Humanoids can carry objects in a way that no other robots can. 
However, humanoids are built with stronger legs and relatively weaker arms. Leveraging body contact to hold and lift heavy objects is essential. Human does this all the time, such as leaning an object on the torso or holding objects on the shoulder. This behavior allows a human to carry more weight without fatiguing their arms as most of the weights are supported by body structure and legs. This clever leverage on contact is potentially transferable to humanoids.

The HRP-4 \cite{AirBus} has achieved a bracket-assembly operation in an aircraft manufacturing task through multi-contact planning and control.


\subsection{State Estimation for Humanoids}

The ability to recognize the robot's ego state in its environment is the first step for planning subsequent actions. State estimation solves this problem by fusing all the sensory data together to form a spatial view of the world. State estimation could use some prior knowledge, such as the map of the room, building, or city. The sensory data may come from proprioception, inertia measurement unit, camera, lidar, force sensor, etc. The goal is to get the state of the robot relative to objects and the environment. The state could contain the position, velocity, contact, etc. A common way to achieve this is through the Kalman filter. Factor Graph has become popular in recent years. Optimization-based estimation became a main trend. Learning methods that adopt auto-regressive mechanisms have an internal latent state that represents the robot's state. 


\section{Safety Guarantee and Robustness against Uncertainty}
Both robustness and safety are crucial aspects of humanoid robots. Robustness relates to the ability to reach the desired state in the face of disturbances. Safety refers to the ability to avoid conditions that could lead to harmful consequences, either to the robot itself or to the environment. 

Due to the prevalent model uncertainties and sensor unreliability. the model-based methods are sensitive to these errors and need improving in robustness. Many mathematical methods are proposed. For example, control Lyapunov function \cite{Reher2021ControlLF} stabilizes the robot walking. Formal methods \cite{Gu_push, Gu_STL} use specifications to describe robust walking tasks, therefore providing a formal guarantee of task completion.
%is the dependence on an accurate model. Uncertainty in the model and estimation may cause errors and failures. However, these methods suffer from dynamic environments and sensor unreliability that are difficult to model precisely. 
Reinforcement learning techniques achieved unprecedented robustness through domain randomization \cite{domain_randomization}. Exposing the robot to environments with diverse physical properties helps form a more robust policy and bridges the sim-to-real gap. 


To achieve safety for humanoid robots, one of the most important aspects is collision avoidance. Control barrier function \cite{CBF_humanoid} is used to enforce strict constraints on self-collision. \cite{Fabrics_WBC, RMP} use kinodynamic fabrics and Riemannian motion policy to fuse collision avoidance tasks together with other tracking tasks. \cite{gu2024robustlocomotionbylogic} use learned kinematic reachability to avoid self-collision between legs. 
Another way is to leverage control strategies to improve compliance \cite{DCC}. 
Another way is to leverage physical intelligence. \cite{Punyo} uses a soft material to absorb contact force. Having transparency and back-drivability built into the actuator \cite{SEA} or transmission \cite{AMBIDEX} also improves safety. In addition, as mentioned in Sec.~\ref{sec:sensing}, sensing capability \cite{cheng2019robotskin} can help mitigate unsafe operations. 

Hybrid methods that blend safety and robustness are also proposed.  \cite{Nguyen_CBF_stone} combines CLF and CBF in a single quadratic program, namely CLF-CBF-QP, to provide robustness and safety simultaneously. Combining the robustness of RL and safety from MPC \cite{SafeRL_MPC} is also a great way. 

In case of failure, the ability to endure and recover from a fall is key to humanoid robots. While many humanoids are equipped with the ability to react to external perturbations using either hip, ankle, or stepping strategy, most don't have the ability to get back up on stand after a fall. Fall detection \cite{mungai2023fall}, fall reaction \cite{gu2024robustlocomotionbylogic}, fall damage reduction \cite{fall_protect_survey}, and fall recovery \cite{fall_recovery} are key components for humanoid as failures are hard to rule out in a dynamical humanoid system that is inherently unstable. Stand-up from a random state after a fall is an important subject. Along this line, \cite{AR_fall_recovery} shows a recovery motion learned by RL after an unexpected trip. \cite{fall_recovery} showed using the learning-based method to stand up, leveraging contact from the ground.

==> figures/category_tree.tex <==
\tikzstyle{my-box}=[
    rectangle,
    draw=hidden-draw,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
]
\tikzstyle{leaf}=[my-box, minimum height=1.5em,
    fill=white!70!red, text=black, align=left,font=\scriptsize,
    inner xsep=2pt,
    inner ysep=4pt,
]
\begin{figure*}[t]
\centering
\resizebox{\textwidth}{!}
{
    \begin{forest}
        forked edges,
        for tree={
            grow=east,
            reversed=true,
            anchor=base west,
            parent anchor=east,
            child anchor=west,
            base=left,
            font=\small,
            rectangle,
            draw=hidden-draw,
            rounded corners,
            align=left,
            minimum width=4em,
            edge={darkgray, line width=1pt},
            % s sep=3pt,
            inner xsep=2pt,
            inner ysep=3pt},
            ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            where level=1{text width=6em,font=\scriptsize,}{},
            where level=2{text width=7em,font=\scriptsize,}{},
            where level=3{text width=7em,font=\scriptsize,}{},
            where level=4{text width=8em,font=\scriptsize,}{},
        [Humanoid Loco-manipulation, ver, 
            [Background of \\ Humanoid Robot \\ (Sec.~\ref{sec:background})
                [{Locomotion and Navigation~\cite{gong2019feedback, huang_cassie_navigation},
                Whole-body Manipulation~\cite{Punyo, WAM_Justin}, Loco-manipulation~\cite{seo2023deep, Murooka_Pattern}}, leaf, text width=33em]
            ]
            [Tactile Sensing \\ (Sec.~\ref{sec:sensing})
                [{Tactile Hand~\cite{yuan2017gelsight, lambeta2020digit}, Whole-body Tactile~\cite{maiolino2013flexible, cheng2019robotskin, Punyo}, Tactile Foot~\cite{xiaofeng_foot, guadarrama2018enhancing}}, leaf, text width=33em]
            ]
            [Traditional Planning \\ and Control
                [Multi-Contact Planning  \\ (Sec.~\ref{sec:contact_planning}), text width=8em
                    [Contact Planning, text width=9em
                        [{Optimization-based~\cite{manchester2020variational,posa2016optimization,mastalli2016hierarchical},
                        Sampling-based~\cite{Murooka_Search,escande2013planning,HutterScience_locomanip}, Learning-based~\cite{lin2019efficient,interdiff}},leaf, text width=25em]
                    ]
                    [Whole-body Pose Planning, text width=9em
                        [{Maximizing interaction forces~\cite{TORO_push}, Perturbation resistance~\cite{Orsolino_FWP}}, leaf, text width=25em]
                    ]
                ]
                [Model Predictive Control \\ (Sec.~\ref{sec:planning}), text width=8em
                    [Model Selection, text width=9em
                        [{Simplified Model~\cite{henze2014posture,li2023dynamic}, Whole-body Model~\cite{koenemann2015whole,penco2019multimode}, Mixed-fidelity Model~\cite{MIT_MHPC,li2021model}},leaf, text width=25em]
                    ]
                    [Speedup Strategies, text width=9em
                        [{Warm Start~\cite{Memmo_2021}, Sampling~\cite{suh2022differentiable}, Structure Exploitation~\cite{vanroye2023fatrop}, Linearization~\cite{zhakatayev_successive_2017}},leaf, text width=25em]
                    ]
                ]
                [Whole-body Control \\ (Sec.~\ref{sec:control}), text width=8em
                    [Closed-form Approaches, text width=9em 
                        [{Inverse Dynamics Control~\cite{sentis_humanoid_prioritization, Mistry2010}, Operational-Space Control~\cite{Sentis2007, mistry_OSC_2008}, Stack of \\Tasks~\cite{SoT_unilateral}},leaf, text width=25em]
                    ]
                    [Optimization Approaches, text width=9em 
                        [{Hierarchical QP~\cite{bellicoso_perception-less_2016, Escande_HQP_humanoid}, Weighted QP~\cite{koolen2016design, siyuan_JFR, Kuindersma2016, hopkins2015compliant}}, leaf, text width=25em]
                    ]
                ]
            ]
            [Learning-based \\ Approaches
                [Skill Learning (Sec.~\ref{sec:learning}), text width=8em
                    [Reinforcement Learning (RL)\\ (Sec.~\ref{sec:RL}) , text width=9em
                        [{Curriculum Learning~\cite{pmlr-v100-xie20a}, Curiosity~\cite{Curiosity-schwarke23a,zhang2024wococo}, Constrained RL~\cite{reward_constraint_RL}},leaf, text width=25em]
                    ]
                    [Imitating Learning (IL) from \\ Robot Experience (Sec.~\ref{sec:expert}), text width=9em
                        [{BC-RNN~\cite{seo2023deep}, IRL~\cite{wu2023infer}, ACT \cite{humanplus, cheng2024tv}}, leaf, text width=25em]
                    ]
                    [Imitation Learning (IL) from \\ Human Data (Sec.~\ref{sec:human}), text width=9em
                        [{GAIL~\cite{gail_locomotion}, RL motion imitation \cite{peng2018sfv}, AMP \cite{AMP}},leaf, text width=25em]
                    ]
                    [Hybrid Methods \\ (Sec.~\ref{sec:combine_method}), text width=9em
                        [{RL+IL~\cite{humanoid_parkour_learning, transformer_digit_RL}, IL+RL~\cite{IFM_quad,Smith2023LearningAA}, Track Reference~\cite{MIMOC, Batke_SRBD_RL, li2023robust, LearnCDM2020}, \\Augment Reference~\cite{Ijspeert_2002, Xie_2018_Cassie, singh2023Access, OPT-Mimic, VictorIROS2022NeuralAdaptation}},leaf, text width=25em]
                    ]
                    [Versatile Skill Learning \\ (Sec.~\ref{sec:skill_composition}), text width=9em
                        [{MOE~\cite{soccer_MOE,basket_ball_starke}, Motion Representations~\cite{Levine_latentRL, li2024fld}, Goal Representation~\cite{cheng2024expressive},\\ \cite{he2024omnih2o}, State Transition Representation~\cite{Hester2010, wu2022daydreamer, mazzaglia2024multimodalfoundationworldmodels, shi2024efficientmodelbasedapproachlearning,hansen2024worldmodelsvisual}},leaf, text width=25em]
                    ]
                ]
                [Foundation Models \\ (Sec.~\ref{sec:foundation_model}), text width=8em
                    [LLMs and VLMs for \\ Humanoids (Sec.~\ref{sec:foundation_model_for_humanoid}), text width=9em
                        [{Figure AI \cite{FigureVideo}, OmniH2O~\cite{he2024omnih2o}, Harmon~\cite{jiang2024harmon}},leaf, text width=25em]
                    ]
                    [Humanoid Foundation \\ Models (Sec.~\ref{sec:humanoid_foundation_model}), text width=9em
                        [{NVIDIA GR00T~\cite{NVIDIAGR00T}, Human VLA~\cite{xu2024humanvla}}, leaf, text width=25em]
                    ]
                ]
            ]
        ]
    \end{forest}
}
\caption{This survey begins by defining relevant concepts of humanoid robots and their locomotion and manipulation capabilities. Centered around achieving whole-body loco-manipulation tasks, the core of this survey delves into two main categories of methods: the traditional planning and control approaches, such as contact planning, motion planning, and control, as well as the emerging learning-based approaches, including skill learning and foundation models. In addition, this survey highlights whole-body tactile sensing as a crucial modality to achieve contact-rich loco-manipulation.}
\label{fig:framework}
\end{figure*}

% [Humanoid Robot, text width=8em
                %     [{e.g. R3M~\cite{nair2022r3m}, SayCan~\cite{Ahn2022DoAI}, Inner Monologue~\cite{huang2022inner}, VoxPoser~\cite{VoxPoser2023}, Mahmoudieh et al.~\cite{mahmoudieh2022zeroshot}}, leaf, text width=30em]
                % ]
                % [Locomotion and Navigation, text width=8em
                %     [{e.g. NL2TL~\cite{chen2023nl2tl}, Chen et al.~\cite{Chen2023}}, leaf, text width=30em]
                % ]
                % [Whole-body Manipulation, text width=8em
                %     [{e.g. ProgPrompt~\cite{progprompt2023}, Code-as-Policy~\cite{codeaspolicies2022}, ChatGPT-Robotics \cite{vemprala2023chatgpt}}, leaf, text width=30em]
                % ]
                % [Loco-Manipulation, text width=8em
                %     [{e.g. RT-1~\cite{RT12023}, RT-2~\cite{rt22023arxiv}, RT-X~\cite{padalkar2023rtx}, PACT~\cite{Bonatti2023}, Xiao et al.~\cite{Xiao2022}, Radosavovic et al.~\cite{Radosavovic2022}, LATTE~\cite{Bucker2023}}, leaf, text width=30em]
                % ]

==> related_survey.tex <==
\subsection{Summary of Previous Surveys}
This survey is related to survey papers in humanoid robotics \cite{humanoid_reference, humanoid_survey_IJAS}, and to the topics of model-based planning \cite{MPC_survey} and control~\cite{Wensing_survey_TRO}, and learning-based methods \cite{Gams2022}. We summarize a list of previous surveys on humanoid loco-manipulation and highlight the differences from our survey paper:
% , learning-based methods for legged robots~\cite{ha2024learningbased}, and foundation models for robotics~\cite{Robots_via_Foundation_Models, firoozi2023foundation}
% A list of other surveys on similar topics that appeared in IJRR or other journals in the past 10 years, and a discussion of differences: why do we need a new RP on this topic?

\textit{Humanoid Robotics: A Reference, 2019} (\cite{humanoid_reference})
\begin{itemize}
    \item This reference book covers the vast areas of humanoid robotics, including mechanical design, modeling, motion planning, and whole-body control. However, this book lacks a connection with more recent research on learning-based methods.
    \item Our study provides not only state-of-the-art model-based planning and control methods but also covers a timely overview of learning-based loco-manipulation methods.
\end{itemize}

\textit{Optimization-based Control for Dynamic Legged Robots, 2022} (\cite{Wensing_survey_TRO}) 
\begin{itemize}
    \item This seminal survey summarizes the model-based control techniques for legged robots, with a focus on optimization-based methods. The survey details problem formulations for predictive control and reactive control.
    \item Our study is distinguished by concentrating on humanoid robots and their loco-manipulation capability. Within this specific focus, we review a wider range of methods for planning and control, including search and learning methods, beyond optimization-only ones.
    \item While learning-based methods are discussed in \cite{Wensing_survey_TRO}, they are not the primary focus. In contrast, our paper will extensively overview learning-based methods.
\end{itemize}

\textit{Model Predictive Control of Legged and Humanoid
Robots: Models and Algorithms, 2023} (\cite{MPC_survey})
\begin{itemize}
    \item This survey provides a review of recent progress in the theory, implementation, and application of MPC techniques to legged and humanoid robots.
    \item While our paper also discusses MPC as the state-of-the-art technique for motion planning, we overview a comprehensive list of both planning and control problems for loco-manipulation, where MPC serves as an individual module of such a planning-control framework.
\end{itemize}

\textit{Advancements in Humanoid Robots: A Comprehensive Review and Future Prospects, 2024} (\cite{humanoid_survey_IJAS})
\begin{itemize}
    \item This survey presents mechanical design, applications, and challenges of humanoid robots, with a brief overview of algorithmic methodologies for planning and control.
    \item Our study is algorithm-driven. The mechanical design and applications are not our focus. Instead, we provide more detailed explanations for both model-based and learning-based methods. %and focus less on robot mechanical design.
\end{itemize}

% \textit{From the State of the Art of Assessment Metrics Toward Novel Concepts for Humanoid Robot Locomotion Benchmarking, 2020} \cite{RAL_humanoid_benchmark}
% \begin{itemize}
%     \item This survey summarizes the most popular humanoid tasks and the evaluation metric of these tasks. 
%     \item Our paper is more methodology-focused and concerns more about how to achieve these tasks.
% \end{itemize}

% \textit{Legged Robots for Object Manipulation: A Review, 2023} \cite{Gong2023LeggedRF}
% \begin{itemize}
%     \item This survey summarizes diverse approaches that multi-legged robots can manipulate objects to achieve tangible goals in human-centric environments.
%     \item Distinguished from this work, our work focuses on humanoid robots, which have a more morphologically suitable form in human-centric environments.
% \end{itemize}

\textit{Manipulation Learning on Humanoid Robots, 2022} (\cite{Gams2022})
\begin{itemize}
    \item This survey focuses on humanoid dual-arm manipulation tasks achieved using the imitation learning (IL) paradigm.
    \item Our study is distinct in terms of both tasks and methodologies. For the task of interest, our study focuses on simultaneous locomotion and manipulation, a task more challenging but less explored compared to traditional manipulation in a stationary set-up. For the methodologies, we provide both traditional motion planning and control as well as more recent learning-based methods, including reinforcement learning (RL) and IL. 
\end{itemize}

\textit{Teleoperation of Humanoid Robots: A Survey, 2023} (\cite{TRO_teleop_survey})
\begin{itemize}
    \item This survey focuses on teleoperation, a specific pipeline that enables versatile humanoid skills.
    \item Our paper provides a broader view and discusses four different data sources that enable versatile humanoid skills, including not only teleoperation, but also robot policy execution, human motion capture, and human video data.
\end{itemize}

Distinct from all the survey papers above, which focus on a few particular areas of humanoid robots, our paper aims to present a broader overview, covering planning, control, and learning topics, including RL, IL, and foundation models. These learning-based approaches provide fundamentally new insights, augment the loco-manipulation capabilities enabled by traditional model-based approaches, and meet the current trends of humanoid robots within both academia and industry. 
%A unique angle this survey holds is the particular emphasis on methods that achieve loco-manipulation behaviors for humanoid robots.
